Direct Post-Training Preference Alignment for Multi-Agent Motion Generation Models Using Implicit Feedback from Pre-training Demonstrations

Recent advancements in LLMs have revolutionized motion generation models in embodied applications. While LLM-type auto-regressive motion generation models benefit from training scalability, there remains a discrepancy between their token prediction objectives and human preferences. As a result, models pre-trained solely with token-prediction objectives often generate behaviors that deviate from what humans would prefer, making post-training preference alignment crucial for producing human-preferred motions. Unfortunately, post-training alignment requires extensive preference rankings of motions generated by the pre-trained model, which are costly to annotate, especially in multi-agent settings. Recently, there has been growing interest in leveraging pre-training demonstrations to scalably generate preference data for post-training alignment. However, these methods often adopt an adversarial assumption, treating all pre-trained model-generated samples as unpreferred examples. This adversarial approach overlooks the valuable signal provided by preference rankings among the model's own generations, ultimately reducing alignment effectiveness and potentially leading to misaligned behaviors. In this work, instead of treating all generated samples as equally bad, we leverage implicit preferences encoded in pre-training demonstrations to construct preference rankings among the pre-trained model's generations, offering more nuanced preference alignment guidance with zero human cost. We apply our approach to large-scale traffic simulation and demonstrate its effectiveness in improving the realism of pre-trained model's generated behaviors, making a lightweight 1M motion generation model comparable to SOTA large imitation-based models by relying solely on implicit feedback from pre-training demonstrations, without additional post-training human preference annotations or high computational costs.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> old_sections/conclusion.tex <==
\vspace{-1em}
\section{Conclusion}
\vspace{-1em}

In this work, we presented a video-only, preference-based learning method for solving the visual representation alignment problem. 
We demonstrated that with an aligned visual representation, reward learning via optimal transport feature matching can generate successful robot behaviors with high sample efficiency, and shows strong zero-shot generalization when the visual reward is learned on a different embodiment than the robot’s.
% Across experiments in X-Magical and in robotic manipulation, RAPL’s reward consistently generates preferred robot behaviors with high sample efficiency, and shows strong zero-shot generalization when the visual reward is learned on a different embodiment than the robot’s.

% \textbf{Limitations \& Future Work.} 
\rb{
% There are several limitations and exciting future directions.
% we focused on robotic experiments in simulation to thoroughly investigate our approach and control for confounds. 
% One limitation of our work is that are the experiments are conducted in simulations so we could control for confounds. 
Although in this work we focused on controlled simulation experiments, future work should validate RAPL with real human feedback and robotic hardware experiments. 
Though our method shows better sample efficiency than RLHF, asking humans for preference queries should be done strategically (e.g., via active learning), should be robust to noisy feedback, and could be improved by leveraging multi-modality (e.g., preferences and language feedback)}. 
% We are interested in using multi-modal human feedback--such as pairing preferences and language explanations of the preferred and disliked behaviors--to make each sample from the human more informative and enable faster and more generalizable visual representation alignment. 
% for learning more generalizable visual representation and reward to improve sample efficiency. 
% Furthermore, we currently decouple the representation and visual reward learning from policy learning, which could potentially suffer from high distribution shift. 
While our current approach was an offline fine-tuning method, future work onto \textit{online} visual reward fine-tuning from human feedback is an exciting direction. \rb{Finally, incorporating feedback from multiple humans (e.g., crowd-sourced multimodal preferences) are also an exciting future direction.}

% Furthermore, we propose a novel visual reward based on recent advances in optimal transport \citep{villani2009optimal} which incentivizes the robot to stay in-distribution of the human's \textit{aligned} visual embedding distribution during policy optimization. 
%\abnote{@Thomas -- lets put some discussion / limitations in here. e.g., we were still just in simulation and we didn't use actual human queries, we can do active learning to show humans triplets that are maximally informative for representation learning.}

==> old_sections/experiments.tex <==
\section{Experimental Design }

We design a series of experiments to investigate RAPL's ability to learn visual rewards and generate preferred robot behaviors. 
% We first detail the experimental design and then present our simulation environments and results. 
% want to study three questions: 1) \textit{Does RAPL's visual reward yield robot policies that are aligned with end-user preferences?} and 2) \textit{How much does an aligned visual representation matter for generating preferred robot behaviors?}, and 3) \textit{What sample complexity gains does our method achieve compared to direct reward prediction?} 

% \subsection{Experimental Design}

\textbf{Preference Dataset: $\tilde{S}_{\reph}$.} While the ultimate test is learning from real end-user feedback, in this work we use a simulated human model as a first step. This allows us to easily ablate the size of the preference dataset, and gives us privileged access to $\rewh$ for direct comparison.
In all environments, the simulated human constructs the preference dataset $\tilde{S}_{\reph}$ by sampling triplets of videos uniformly at random from the set\footnote{To minimize the bias of this set on representation learning, we construct $\tilde{\Xi}$ such that the reward distribution of this set under  $\rewh$, is approximately uniform. Future work should investigate the impact of this set further, e.g., \citep{sadigh2017active}.} of video observations $\tilde{\Xi} \subset \Xi$, and then ranking them with their reward $\rewh$ as in  \autoref{eq:representation_alignment_loss}. 

\textbf{Independent \& Dependent Measures.} Throughout our experiments we vary the \textit{visual reward signal} used for robot policy optimization and the \textit{preference dataset size} used for representation learning. 
% The reward signal includes varying the visual representation, how the reward is trained, etc. 
We measure robot task success as a binary indicator of if the robot completed the task with high reward $\rewh$. 
% The success rate is the 

\textbf{Controlling for Confounds.} 
Our ultimate goal is to have a visual robot policy, $\policyr$, that takes as input observations and outputs actions. 
However, to rigorously compare policies obtained from different visual rewards, we need to disentangle the effect of the reward signal from any other policy design choices, such as the input encoders and architecture. 
To have a fair comparison, we follow the approach from \citep{zakka2022xirl, kumar2023graph} and input the privileged ground-truth state into all policy networks, but vary the visual reward signal used during policy optimization. 
Across all methods, we use an identical reinforcement learning setup and Soft-Actor Critic for training \citep{haarnoja2018soft} with code base from \citep{zakka2022xirl}.
% All policies are optimized via Soft-Actor Critic reinforcement learning \citep{} and the policy network is a 3-layer MLP with \abnote{activations}. 

% to eliminate the confounding effect induced by observation.
%The state representation follows from \citep{zakka2022xirl} with minor modifications for our settings. 

In Section~\ref{sec:in-domain-results}, we first control the agent's embodiment to be consistent between both representation learning and robot optimization (e.g., assume that the robot shows video triplets of itself to the human and the human ranks them). 
In Section~\ref{sec:cross-domain-results}, we relax this assumption and consider the more realistic cross-embodiment scenario where the representation learning is performed on videos of a different embodiment 
% a dataset from a different embodiment 
% (e.g., human shows themselves doing the task in a way that they like and a way that they do not) 
than the robot's. For all policy learning experiments, we use $10$ expert demonstrations as the demonstration set $\mathcal{D}_+$ for generating the reward (for details on this see Appendix~\ref{app:OT}).


% if we want to control the true ``state'' of the world that generates the visual observations, and only vary the ground-truth human's preference. 
% This means we first do experiments in-domain, assuming that the robot and the human operate on the same embodiment. This enables us to determine which method can learn the visual preferences, all other things held constant. 

 

% \textbf{Representation alignment.} 
% We want to validate the effectiveness of the learned visual reward and the induced robot policy compared to the human's policy. 
% To fully validate both, 
% We manually design state based ``ground truth" reward function as a ``simulated judge'' to construct the $\tilde{S}_{\reph}$ which contains $150$ preference triplets. 

\section{Results: From Representation to Behavior Alignment}
\label{sec:in-domain-results}

We first experiment in the toy X-Magical environment \citep{zakka2022xirl}, and then move to the realistic IsaacGym simulator. 

\subsection{X-Magical}
\label{subsec:in-domain-xmagical}

\begin{wrapfigure}{r}{0.41\textwidth}
    \vspace{-0.5cm}
    \includegraphics[width=0.41\textwidth]{figs/sim_environments_2.png}
    \vspace{-0.7cm}
  \caption{X-Magical \& IsaacGym tasks.}
  \vspace{-0.5cm}
  \label{fig:x-magical-env}
\end{wrapfigure}


\textbf{Tasks.}  We design two tasks inspired by kitchen countertop cleaning. The robot always has to push objects to a goal region (e.g., trash can), shown in pink at the top of the scene in \autoref{fig:x-magical-env}. In the \textbf{avoiding} task, the end-user prefers that the robot and objects never enter an \textit{off-limits zone} during pushing (blue box in left \autoref{fig:x-magical-env}).
% where the robot needs to push the object (red square) towards a static goal region (light red region) without entering a disfavored region (light blue region). 
In the \textbf{grouping} task, the end-user prefers that objects are always pushed \textit{efficiently together} (instead of one-at-a-time) towards the goal region (center, \autoref{fig:x-magical-env}).

\textbf{Privileged State \& Reward.}
For \textbf{avoiding}, the true state $s$ is 7D: planar robot position ($p_\robot \in \mathbb{R}^2$) and orientation ($\theta_\mathrm{R}$),  planar position of the object ($p_{\mathrm{obj}}\in \mathbb{R}^2$), distance between goal region and object, ($d_{\mathrm{obj2goal}}$), and distance between the off-limits zone and the object ($d_{\mathrm{obs2obj}}$). The human's reward is: $\rewh_{\mathrm{avoid}}(s) = - d_{\mathrm{goal2obj}} - 2\cdot \mathbb{I}(d_{\mathrm{obs2obj}} < d_{\mathrm{safety}})$, where $d_{\mathrm{safety}}$ is a safety distance and $\mathbb{I}$ is an indicator function giving $1$ when the condition is true.
For \textbf{grouping}, the state is 9D: $s := (p_\robot, \theta_\robot$, $p_{\mathrm{obj^1}}, p_{\mathrm{obj^2}}, d_{\mathrm{goal2obj^1}}$, $d_{\mathrm{goal2obj^2}})$. The human's reward is: $\rewh_{\mathrm{group}}(s) = - \max(d_{\mathrm{goal2obj^1}}, d_{\mathrm{goal2obj^2}}) - ||p_{\mathrm{obj^1}} - p_{\mathrm{obj^2}}||_2$.

\textbf{Baselines.} We compare our visual reward, \rapl, against (1) \gt, an oracle policy obtained under $\rewh$, (2) \rlhf, which is vanilla preference-based reward learning \citep{christiano2017deep, brown2019extrapolating} that directly maps an image observation to a scalar reward, and (3) \tcc \citep{zakka2022xirl,kumar2023graph} which finetunes a pre-trained encoder via temporal cycle consistency constraints using 500 task demonstrations and then uses L2 distance between the current image embedding and the goal image embedding as reward. We use the same preference dataset with $150$ triplets for training RLHF and RAPL. 

\textbf{Visual model backbone.} We use the same setup as in \citep{zakka2022xirl} with the ResNet-18 visual backbone \citep{he2016deep} pre-trained on ImageNet. The original classification head is replaced with a linear layer that outputs a $32$-dimensional vector as our embedding space, $\Phi_\robot := \mathbb{R}^{32}$. The TCC representation model is trained with 500 demonstrations using the code from \citep{zakka2022xirl}. Both RAPL and RLHF only fine-tune the last linear layer. All representation models are frozen during policy learning.

\textbf{Hypothesis}. \textit{\rapl is better at capturing preferences \textit{beyond} task progress compared to direct reward prediction \rlhf or \tcc visual reward, yielding higher success rate.} 

% =========== XMAGICAL ============= %
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{figs/xmagical_indomain_reward_new.pdf}
    \vspace{-1em}
    \caption{\textbf{X-Magical.} (left \& right) examples of preferred and disliked videos for each task. (center) reward associated with each video under each method. RAPL's predicted reward follows the GT pattern: low reward when the behavior are disliked and high reward when the behavior are preferred. RLHF and TCC assign high reward to disliked behavior (e.g., (D)). }
    \vspace{-1em}
    \label{fig:xmagical_indomain_reward}
\end{figure*}

% =========== XMAGICAL ============= %
% \begin{wrapfigure}{r}{0.8\textwidth}
%     \vspace{-0.5cm}
%     \includegraphics[width=0.8\textwidth]{figs/xmagical_indomain_policy.pdf}
%     \vspace{-0.8cm}
%   \caption{\textbf{X-Magical.} Policy evaluation success rate during policy learning. Colored lines are the mean and variance of the evaluation success rate.}
%   %\vspace{-0.5cm}
%   \label{fig:xmagical_indomain_policy}
% \end{wrapfigure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{figs/xmagical_indomain_policy.pdf}
    \vspace{-1em}
    \caption{\textbf{X-Magical.} Policy evaluation success rate during policy learning. Colored lines are the mean and variance of the evaluation success rate. RAPL can match GT in the \textbf{avoiding} task and outperforms baseline visual rewards in \textbf{grouping} task.}
    \vspace{-0.5em}
    \label{fig:xmagical_indomain_policy}
\end{figure*}

\textbf{Results.} 
Figure~\ref{fig:xmagical_indomain_reward} shows the rewards over time for three example video observations in the \textbf{avoid} (left) and \textbf{group} task (right). Each video is marked as preferred by the end-user's ground-truth reward or disliked. 
% \rapl rewards withe the baseline visual rewards and the \gt rewards for the avoiding task (left) and the grouping task (right). 
Across all examples, \rapl's rewards are highly correlated with the \gt rewards: when the behavior in the video is disliked, then reward is low; when the behavior is preferred, then the reward is increasing. \tcc's reward is correlated with the robot making spatial progress (i.e., plot (E) and (F) where observations get closer to looking like the goal image), but it incorrectly predicts high reward when the robot makes spatial progress but violates the human's preference ((C) and (D) in \autoref{fig:xmagical_indomain_reward}). \rlhf performs comparably to \rapl, with slight suboptimality in scenarios (C) and (D). 
Figure~\ref{fig:xmagical_indomain_policy} shows the policy evaluation success rate during RL training with each reward function (\rb{solid line is the mean, shaded area is the standard deviation, over 5 trials with different random seeds.}). Across all environments, \rapl performs comparably to \gt (\textbf{avoid} success: $\approx80\%$, \textbf{group} success: $\approx60\%$) and significantly outperforms all baselines with better sample efficiency, RAPL takes 10 epochs to reach 70\% success rate in the \textbf{avoid} task (GT requires 100) and takes 100 epochs to reach 40\% success rate in the \textbf{avoid} task (GT requires 150), supporting our hypothesis.
\vspace{-1em}

\subsection{Robot Manipulation}
\label{subsec:in-domain-manipulation}

In the X-Magical toy environment, RAPL outperformed progress-based visual rewards, but direct preference-based reward prediction was a competitive baseline. Moving to the more realistic robot manipulation environment, we want to 1) disentangle the benefit of our fine-tuned representation from the optimal transport reward structure, and 
% is the benefit of \rapl attributed by optimal transport only?
2) understand if our method still outperforms direct reward prediction in a more complex environment?

\label{subsubsec:manipulation-setup}
\textbf{Task.} We design a robot manipulation task in the IsaacGym physics simulator \citep{makoviychuk2021isaac}. We replicate the tabletop \textbf{grouping} scenario, where a Franka robot arm needs to learn that the end-user prefers objects be pushed \textit{efficiently together} (instead of one-at-a-time) to the goal region (light blue region in right of \autoref{fig:x-magical-env}). 

\textbf{Privileged State \& Reward.}
The state $s$ is 18D: robot proprioception ($\theta_{\mathrm{joints}}\in \mathbb{R}^{10}$), 3D object positions
($p_{\mathrm{obj^{1,2}}}$), and object distances to goal ($d_{\mathrm{goal2obj^{1,2}}}$). The \textbf{grouping} reward is identical as in Section~\ref{subsec:in-domain-xmagical}. 

\textbf{Baselines.} In addition to comparing \rapl against (1) \gt and (2) \rlhf, we ablate the \textit{representation model} but control the \textit{visual reward structure}. We consider five additional baselines that all use optimal transport-based reward but operate on different representations: (3) \mvpot which learns image representation via masked visual pre-training; \prb{(4) \mvpotfinetune, which fine-tunes MVP representation  using images from the task environment; (5) \rtm, which is an off-the-shelf ResNet-18 encoder \citep{nair2022r3m} pre-trained on the Ego4D data set \citep{grauman2022ego4d} via a learning objective that combines time contrastive learning, video-language alignment, and a sparsity penalty; (6): \imagenet, which is a ResNet-18 encoder pre-trained on ImageNet;} (7) \tccot \citep{dadashi2020primal} which embeds images via the TCC representation trained with 500 task demonstrations. We use the same preference dataset with $150$ triplets for training RLHF and RAPL.



\textbf{Visual model backbone.} All methods except MVP-OT and Fine-Tuned-MVP-OT share the same ResNet-18 visual backbone and have the same training setting as the one in the X-Magical experiment. MVP-OT and Fine-Tuned-MVP-OT use a off-the-shelf visual transformer \citep{xiao2022masked} pre-trained on the Ego4D data set \citep{grauman2022ego4d}. All representation models are frozen during policy learning.


\textbf{Hypotheses}. \textbf{H1:} \textit{\rapl's higher success rate is driven by its aligned visual representation}. \textbf{H2:} \textit{\rapl outperforms \rlhf with lower amounts of human preference queries}.


% ======== IN-DOMAIN: MANIPULATION ======= %
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{figs/franka_OT_rew_indomain_new.pdf}
    \caption{\textbf{Manipulation. }   
    (center) Expert, preferred, and disliked video demo.
    (left) reward associated with each video under each method. RAPL's predicted reward follows the GT pattern. RLHF assigns high reward to disliked behavior.
    % Across both types of demos, \rapl matches the same reward trends as \gt, while other methods struggle to disambiguate. 
    (right) OT coupling for each representation. Columns are embedded frames of expert demo. Rows of top matrices are embedded frames of preferred demo; rows of bottom matrices are embedded frames of disliked demo. Peaks exactly along the diagonal indicate that the frames of the two videos are aligned in the latent space; uniform values in the matrix indicate that the two videos cannot be aligned (i.e., all frames are equally ``similar’’ to the next). RAPL matches this structure: diagonal peaks for expert-and-preferred and uniform for expert-and-disliked, while baselines show diffused values no matter the videos being compared.}
    \label{fig:franka_OT_rew_indomain}
    \vspace{-1em}
\end{figure*}

% ======== IN-DOMAIN: MANIPULATION ======= %

\begin{wrapfigure}{r}{0.5\textwidth}
    \vspace{-0.5cm}
    \includegraphics[width=0.5\textwidth]{figs/franka_success_v_reward_all_baselines.pdf}
    \vspace{-0.8cm}
  \caption{\textbf{Manipulation.} Success rate during robot policy learning for each visual reward. }
  \vspace{-0.2cm}
  \label{fig:franka_success_v_reward}
\end{wrapfigure}


\textbf{Results: Reward prediction \& policy learning.} 
In the center of Figure~\ref{fig:franka_OT_rew_indomain} we show three video demos: an expert video demonstration, a preferred video, and a disliked video. 
On the right of Figure~\ref{fig:franka_OT_rew_indomain}, we visualize the optimal transport plan comparing the expert video to the disliked and preferred videos under each visual representation, $\phi_{\rapl}$, $\phi_{\tccot}$, $\phi_{\mvpot}$. Intuitively, peaks exactly along the diagonal indicate that the frames of the two videos are aligned in the latent space; uniform values in the matrix indicate that the two videos cannot be aligned (i.e., all frames are equally ``similar’’ to the next).
\rapl's representation induces precisely this structure: diagonal peaks when comparing two preferred videos and uniform when comparing a preferred and disliked video. 
% The transport plan has peak values along the diagonal when transporting the preferred trajectory's empirical aligned embedding distribution to that of the expert trajectory, indicating high alignment between the two, and has evenly spread values when transporting disliked trajectory's empirical aligned embedding distribution to the expert's, indicating poor alignment between the two. 
Interestingly, we see diffused peak regions in all transport plans under both \tccot and \mvpot representations, indicating their representations struggle to align preferred behaviors and disentangle disliked behaviors.
This is substantiated by the left of Figure~\ref{fig:franka_OT_rew_indomain}, which shows the learned reward over time of preferred video and disliked video. Across all examples, \rapl rewards are highly correlated to \gt rewards while baselines struggle to disambiguate, supporting \textbf{H1}.

Figure~\ref{fig:franka_success_v_reward} shows the policy evaluation history during RL training with each reward function. We see \rapl performs comparably to \gt (succ. rate: $\approx 70\%)$ while all baselines struggle to achieve a success rate of more than $\approx 10\%$ with the same number of epochs.  
It's surprising that \rlhf fails in a more realistic environment since its objective is similar to ours, but without explicitly considering representation alignment. 
To further investigate this, we apply a linear probe on the final embedding and visualize the image heatmap of what each method's final embedding pays attention to in Figure~\ref{fig:attention_map} in the Appendix. 
\rlhf is biased towards paying attention to irrelevant areas that can induce spurious correlations; in contrast \rapl learns to focus on the task-relevant objects and the goal region. 

\begin{wrapfigure}{r}{0.38\textwidth}
    \vspace{-0.5cm} \includegraphics[width=0.38\textwidth]{figs/OT_datasize_exp.png}
    \vspace{-0.6cm}
    \caption{\textbf{Manipulation.} \rapl sample efficiency analysis. RAPL can achieve $\approx$ 45\% success rate with only 25 preference queries.}
    \label{fig:rapl_sample_size_exp}
    \vspace{-0.5cm}
\end{wrapfigure}

\textbf{Results: Sample complexity.} 
We further study the sensitivity of RAPL and RLHF to the preference query dataset size. 
% We study this in the Franka manipulation domain.  
For RLHF, we double the preference query dataset during reward model training to 300 queries (detailed in App. \ref{app:rlhf-with-doubled-data}). Policy performance is improved, indicating that with more feedback data, preference-based reward prediction could yield an aligned policy. Nevertheless, \rapl outperforms \rlhf by $75\%$ with $50\%$ less training data, supporting \textbf{H2}. 
% We are interested in the sample complexity of \rapl for learning a good representation. 
While all the RAPL results above used 150 preference queries to train the representation, we also train a visual representation with 100, 50, and 25 preference queries.  Figure~\ref{fig:rapl_sample_size_exp} shows the success rate of the robot manipulation policy for each version of RAPL. 
We note that \rapl achieves a 45\% success rate even when trained on only 25 preference queries.


% \prb{\textbf{Results: Additional vision model baselines.}  We further studied three additional OT-based reward baselines in the robot manipulation setting described in Appendix~\ref{app:additional baselines}: (1) Fine-Tuned-MVP-OT, which fine-tunes MVP representation using images from the task environment; (2) R3M-OT, which is an off-the-shelf ResNet-18 encoder pre-trained on the Ego4D data set via a learning objective that combines time contrastive learning, video-language alignment, and a sparsity penalty (Nair et al., 2022); (3) ImageNet-OT, which is a ResNet-18 encoder pre-trained on ImageNet. 
% We find that our method significantly outperforms these alternative visual representations in terms of task success.


\subsubsection{Additional Complex Manipulation Task with Visual Distractors}
\label{subsec: multi object push}
% Additional experiments on a more complex robot manipulation task. 
% Per the reviewer’s suggestion, 
Finally, we implemented a more complex robot manipulation task---named \textbf{clutter} in the text and charts---to further validate RAPL’s ability to disentangle visual features that underlie an end-user's preferences. 
We increased the difficulty of the robot manipulation environment described in Section~\ref{subsec:in-domain-manipulation} by introducing more objects to the tabletop and adding visual distractors that are irrelevant to the human's preferences. 
The environment has multiple objects on the table of various colors---red, green, and ``goal-region''-blue---and some of the objects are cubes while others are rectangular prisms. 
The Franka robot arm needs to learn that the end-user prefers to push the rectangular objects (instead of the cube objects) efficiently together (instead of one-at-a-time) to the goal region. 
Color of the objects is a distractor feature. 
Compared to the original \textbf{grouping} manipulation task described above, the Franka arm needs to learn visual representations that can disentangle both semantic preference (grouping) and low-level preference (shape) from RGB images under visual distractors (object color). In addition, the Franka arm needs to learn to grasp the rectangular object first and use that to push the second rectangular object, as it is difficult to directly push the rectangular object stably using the robot finger gripper, thus increasing the task difficulty.
The detailed task description and results are reported in Appendix~\ref{app: multi object push}.
We find that in this more complex manipulation and preference-learning task, \rapl performs comparably to a policy with ground-truth reward (succ. rate: $\approx 65\%$) while all baselines struggle to acheive success rate of more than $\approx 10\%$.


\subsubsection{Spearman’s correlation between GT and learned visual rewards}

\prb{We conducted a quantitative analysis to investigate the relationship between the learned visual reward and the end-user’s ground-truth reward. For the robot manipulation tasks described in Section~\ref{subsec:in-domain-manipulation} (Franka Group), Section~\ref{sec:cross-domain-results} (Kuka Group), and Section~\ref{subsec: multi object push} (Franka Clutter), we computed the average Spearman’s correlation coefficient between the ground-truth reward trajectory and any other approach's reward trajectory across 100 video trajectories. We found that \rapl's learned visual reward shows the strongest correlation to the \gt reward compared to baselines.

\renewcommand{\arraystretch}{1.25}
\begin{table}[h!]
    \centering
    \begin{tabular}{| p{0.77in} | c | c | c | }
    \hline
       & \multicolumn{3}{|c|}{ \textbf{Spearman's Correlation} } \\ \hline 
         & \textbf{Franka Group} (Sec.~\ref{subsec:in-domain-manipulation}) & \textbf{Kuka Group} (Sec.~\ref{sec:cross-domain-results}) & \textbf{Franka Clutter} (Sec.~\ref{subsec:in-domain-manipulation}) \\ \hline
        \rapl & 0.59 &  0.47 & 0.61\\ \hline
        \rlhf & 0.38 &  0.31 & 0.26\\ \hline
        \mvpot &  -0.1&  0.02 & 0.08\\ \hline
        \mvpotfinetuneabbrev &  0.19&  0.02& 0.11 \\ \hline
        \imagenetabbrev &  -0.09 &  0.12 & -0.02\\\hline
        \rtm & 0.03 &  -0.14 &  -0.17 \\ \hline
    \end{tabular}
    \caption{\rb{Spearman's rank correlation coefficient between the \gt reward and each learned reward.}}
    \label{table:Spearman}
\end{table}
}




\section{Results: Zero-Shot Generalization Across Embodiments}
\label{sec:cross-domain-results}

So far, the preference feedback used for aligning the visual representation was given on videos $\obstraj \in \tilde{\Xi}$ generated on the same embodiment as that of the robot. 
However, in reality, the human could give preference feedback on videos of a \textit{different} embodiment than the specific robot's.
% However, in reality, the easiest interface for soliciting preferences could be for the human to directly \textit{show themselves} performing the task in desired and less desired ways. 
% Thus, the preference dataset $\tilde{S}_\human$ used for aligning the representation will be generated on a \textit{different} embodiment than the robot's. 
We investigate if our approach can \textit{generalize} to changes in the embodiment between the preference dataset $\tilde{S}_\human$ and the robot policy optimization. 

% ========== XMAGICAL: CROSS EMBODIMENT =========== %
\begin{figure*}[h]
    \centering
    \vspace{-0.5cm}
    \includegraphics[width=0.85\textwidth]{figs/xmagical_crossdomain_policy.pdf}
    \vspace{-1.5em}
    \caption{\textbf{Cross-Embodiment: X-Magical.} Policy evaluation success rate during policy learning. Colored lines are the mean and variance of the evaluation success rate. RAPL achieves a comparable success rate compared to GT with high learning efficiency, and outperforms RLHF and TCC.}
    \vspace{-1em}
    \label{fig:xmagical_crossdomain_policy}
\end{figure*}

\textbf{Tasks \& Baselines.} We use the same setup for each environment as in Section~\ref{sec:in-domain-results}.


\textbf{Cross-Domain Agents.} In X-Magical, reward functions are always trained on the \textit{short stick} agent, but the learning agent is a \textit{gripper} in \textbf{avoid} and a \textit{medium stick} agent in \textbf{grouping} task. In robot manipulation we train RAPL and RLHF on videos of the \textit{Franka} robot, but deploy the rewards on the \textit{Kuka} robot.

\textbf{Hypothesis.} \textit{\rapl enables zero-shot cross-embodiment generalization of the visual reward compared to other visual rewards.}


% the world may be different when the human and the robot generate data because the two agents do not share the same embodiment. For example, instead of teleoperating the robot, the human may want to show how to do the task on their own. The robot learns its representation and visual reward from this dataset that is generated on the human's embodiment, but then has to optimize this visual reward \textit{on its own} embodiment. 

% \tr{Maybe just highlighting the x-magical and manipulation RL results together here, and put the reward vis in the appendix?}
% \abnote{Yes, I think thats a great idea.}



\textbf{Results.} 
Figure~\ref{fig:xmagical_crossdomain_policy} and  Figure~\ref{fig:kuka_success_v_reward} show the policy evaluation histories during RL training with each reward function in the cross-embodiment X-Magical environment and the manipulation environment. We see that in all cross-embodiment scenarios, \rapl achieves a comparable success rate compared to \gt and significantly outperforms baselines which struggle to achieve more than zero success rate, supporting \textbf{H1}. See more results in App. \ref{app:cross-domain-results}.
% and demonstrate that RAPL’s rewards are highly correlated with the \gt rewards even when deployed on a cross-embodiment robot.


% ========== Manipulation: CROSS EMBODIMENT =========== %
\begin{wrapfigure}{r}{0.5\textwidth}
    \vspace{-0.5cm}
    \includegraphics[width=0.5\textwidth]{figs/kuka_success_v_reward_all_baselines.pdf}
    \vspace{-0.5cm}
  \caption{\textbf{Cross-Embodiment: Manipulation.} Colored lines are the mean and variance of the success rate during policy learning.}
  %\vspace{-0.2cm}
  \label{fig:kuka_success_v_reward}
\end{wrapfigure}



We note an interesting finding in the X-Magical grouping task when the representation is trained on videos of the \textit{short stick} agent, but the learning agent is the \textit{medium stick} agent (see Figure~\ref{fig:xmagical_crossdomain_reward} in Appendix). 
Because the \textit{short stick} agent is so small, it has a harder time keeping the objects grouped together; in-domain results from Section~\ref{sec:in-domain-results} show a success rate of $\approx$ 60\% (see Figure~\ref{fig:xmagical_indomain_policy}). 
In theory, with a well-specified reward, the task success rate should \textbf{increase} when the \textit{medium stick} agent does the task, since it is better suited to push objects together. 
Interestingly, when the \textit{short stick} visual representation is transferred zero-shot to the \textit{medium stick}, we see precisely this: \rapl's task success rate \textbf{improves} by 33\% under cross-embodiment transfer (succ. rate $\approx$ 80\%). 
% The finding that our visual representation can be learned from videos of an embodiment that struggles to do object grouping effectively, but then can be zero-shot transferred to an embodiment that can do the task easily 
This finding indicates that RAPL can learn task-relevant features that can guide correct task execution even on a new embodiment. 



==> old_sections/intro.tex <==
\section{Introduction}

Imagine that a robot manipulator is tasked with cleaning your kitchen countertop. 
To be successful, its reward function should model your preferences: what you think an orderly kitchen countertop looks like (e.g., plates should be stacked by color), how objects should be handled during cleaning (e.g., cups should be moved one-at-a-time but food scraps should be pushed in large groups), and what parts of the countertop should be avoided (e.g., always stay away from the expensive espresso machine).

A long-standing approach to this problem has been through inverse reinforcement learning (IRL), where the robot infers a reward from demonstrations. 
Fundamental work in IRL \citep{abbeel2004apprenticeship, ziebart2008maximum} argues for matching features between the expert and the learner during reward inference, more formally known as optimizing Integral Probability Metrics (IPMs) \citep{sun2019provably, swamy2021moments}. 
While there are many ways to do this matching, optimal transport methods have recently been used to optimize IPMs defined on high-dimensional feature spaces in a principled manner
\citep{villani2009optimal, xiao2019wasserstein, dadashi2020primal, papagiannis2022imitation, luo2023optimal}. 

The question remains, what are good features for the learner to match? While traditional work used hand-engineered features defined on low-dimensional states of the world that the robot could do state estimation on (e.g. object pose) \citep{levine2011nonlinear, finn2016guided}, 
% features were hand-engineered to model what matters, and defined on low-dimensional states of the world that the robot could do state estimation on (e.g. object pose) \citep{levine2011nonlinear, finn2016guided}.
% \tr{I changed the logic in this paragraph.}
% While recent advances in optimal transport \citep{villani2009optimal} enable robots to perform feature matching in a principled way in high dimensional state spaces, key to making this matching work from visual input is a good visual embedding as it directly controls the robot is trying to learn. 
large vision models trained via self-supervised/unsupervised learning promise representations for robotics that directly operate on raw image inputs and capture more nuanced features automatically (e.g., object color and shape) \citep{xiao2022masked, ma2023vip, karamcheti2023language}.
However, automatically extracting relevant visual features that incentivize preferred robot behavior and minimize spurious correlations remains an open challenge \citep{zhang2020learning}. 
% feature matching based visual rewards built on these representations often fail to incentivize desired robot behavior as the representation learning purposefully bypasses human's input on the task of the interest, exacerbating spurious correlations \citep{zhang2020learning}.
Previous works use proxy tasks during representation learning to imbue some prior human knowledge about attributes that are relevant \citep{brown2020safe}, such as assuming access to action labels and doing behavior cloning \citep{haldar2023watch, haldar2023teach} or performing temporal cycle-consistency learning \citep{dadashi2020primal}. 
The former requires additional signals that may be hard to obtain (i.e., actions), while the latter assumes that temporal consistency signal is sufficient to extract what matters to the task, potentially ignoring other features that matter to the demonstrator (e.g., avoiding undesired regions).
% However, some proxy tasks require additional signals that may hard to obtain (e.g., actions) and it's not feasible to know each user's internal attributes a-priori, ultimately leading to misaligned robot behaviors.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{figs/front_fig.pdf}
    \caption{Representation-Aligned Preference-based Learning (RAPL), is an action-free visual representation learning method using easy-to-provide human preference feedback on video demos. Using the human preference triplets, the robot goes from paying attention to the end-effector ($\tilde{\phi}_{\mathrm{H}}^0$) to paying attention to the objects and the goal region ($\tilde{\phi}_{\mathrm{H}}^*$) at the end of alignment. The aligned representation is used to construct an optimal transport-based visual reward for robot behavior learning.}
    \vspace{-1.5em}
    \label{fig:front_fig}
\end{figure*}

Since robots ultimately operate in service of people,
%, instead of building representations through proxy tasks that remove direct feedback from the person,
recent works advocate that the robot should explicitly engage in a \textit{representation alignment process} with the end-user. 
% optimize for representations that capture what matters to the task directly from the end-user. 
These works leverage user feedback such as human-driven feature selection \citep{bullard2018human, luu2019incremental}, interactive feature construction \citep{bobu2021feature, katz2021preference} or similarity-queries \citep{bobu2023sirl} to learn human-centric representations.
% relevant for expressing user preferences. 
However, these approaches either operate on pre-defined feature sets or in low-dimensional state spaces (e.g., positions). %learn human-aligned features
In the visual domain, \rb{\citep{zhang2020learning} uses manually-defined reward signals to learn representations which disentangle high versus low reward images; unfortunately, when the main objective \textit{is} reward learning in the first place, this approach is not feasible.}

% directly use per-image reward signals to align image representation with the human preference encoded in the reward signal, while directly accessing such a preference signal is not practical. 
% Our work utilizes human preference feedback that naturally contains human preference to align robot's visual representations with the end user.

\textit{Instead of hoping to extract human-centric visual representations from demonstration videos via proxy tasks that bypass human input or require action labels per video frame, we propose that robots use easy-to-provide human preference feedback---where the human is asked to compare two (or more) videos---to align their visual representations with what matters to the end-user (Figure~\ref{fig:front_fig}). }
% This feedback is often easier for people to give than kinesthetic teaching or fine-grained feedback \citep{shin2023benchmarks}.

% While demonstrations have been the data of choice for reward learning in the past, an increasingly popular approach is to use preference-based learning \citep{christiano2017deep, sadigh2017active, biyik2018batch, wirth2017survey, brown2019extrapolating, shin2023benchmarks, stiennon2020learning}. Here the human is asked to compare one (or more) trajectories, and then the robot infers a map from ranked trajectories to a scalar reward. This feedback is often easier for people to give than kinesthetic teaching or fine-grained feedback \citep{shin2023benchmarks}.
% \textit{In this work, we propose that robots use easy-to-provide human preference feedback on raw videos to \textit{align} their \textit{visual} representations with the end user, and disentangle what matters for the task.} 

We first formalize the visual representation alignment problem for robotics as a metric learning problem in the human's representation space. 
We then propose \textbf{R}epresentation-\textbf{A}ligned \textbf{P}reference-based \textbf{L}earning (\textbf{RAPL}), a tractable video-only method for solving the alignment problem and learning visual robot rewards via optimal transport. 
Across experiments in X-Magical \citep{zakka2022xirl} and in robotic manipulation, we find that RAPL’s reward consistently generates preferred robot behaviors with high sample efficiency, and shows strong zero-shot generalization when the visual representation is learned on a different embodiment than the robot’s.
% and superior zero-shot generalization when the visual reward is deployed on a new embodiment that is more suitable for the task.


%We introduce \textbf{R}epresentation-\textbf{A}ligned \textbf{P}reference-based \textbf{L}earning (RAPL), a video-only preference-based representation learning approach for vision-based robotics. 




% Specifically, we introduce the first video-only preference-based representation learning approach for fine-tune pre-trained vision models for robotics.
% Furthermore, we propose a novel visual reward based on recent advances in optimal transport \citep{villani2009optimal} which incentivizes the robot to stay in-distribution of the human's \textit{aligned} visual embedding distribution during policy optimization. 
% We call this process of generating aligned robot behaviors from raw visual inputs, \textbf{R}epresentation-\textbf{A}ligned \textbf{P}reference-based \textbf{L}earning (RAPL). 

%the ability of the robot to match the human's preferences hinges on the \textit{alignment} between the robot and human's visual representation.


%representation alignment is becoming increasingly important for robots to interpret the world in the same way as we do.


% Visual robot rewards promise to capture task preferences directly from videos.  
% Self-supervised approaches use task progress inherent in video demonstrations to learn how ``far'' the robot is from completing the task \citep{zakka2022xirl, kumar2023graph, ma2023vip} 
% while other approaches identify task segments and measure distance to these subgoals \citep{sermanet2016unsupervised, tanwani2020motion2vec, shao2020concept, chen2021learning}. 
% However, these approaches fail to model nuanced end-user preferences \textit{during} task execution that go beyond progress (e.g., spatial regions to avoid during movement). 





%In contrast to prior works that rely on hard-to-obtain action labels or using only self-supervised signal, we propose an OT-based visual reward that is trained 
%purely on videos (no action labels needed) that ranked by the \textit{end-user's} preferences. 

% No matter the task, the robot's reward function inherently depends on a \textit{representation}--i.e., the space of \textit{features}--like plate color or scrap grouping.
% Traditionally, these features were hand-engineered and defined on low-dimensional states of the world that the robot could do state estimation on (e.g. object pose) \citep{abbeel2004apprenticeship, ziebart2008maximum, levine2011nonlinear, finn2016guided}, but recently pre-trained vision models \citep{bla} promise representations for robotics that directly operate on raw image inputs and capture more nuanced features automatically (e.g., object color). 
% Key to making these visual representations useful for robotics is the tuning (or training) them via proxy tasks such as behavior cloning \citep{haldar2023watch, haldar2023teach} or temporal cycle-consistency learning \citep{dadashi2020primal}. \abnote{more proxy tasks??} However, all these proxy tasks bypass the human's input on what matters to \textit{them}, leading to spurrious correlations and misaligned robot behaviors. 


%\abnote{TODO: last paragraph which summarizes our results and findings. Something like, ``Across simulation experiments in the X-Magical and IsaacGym environments, we ''}

% In this work, we hypothesize that if a vision-based robot is to optimize for behaviors that are aligned with human preferences, then it should understand the visual world the way that the human does. 
% In other words, the robot's reward should rely on a visual representation that is \textit{aligned} with the human's.
% We leverage preference-based learning paradigm to the visual robot learning domain by developing a sample-efficient visual reward which captures what the human cares about. 

% However, these representations are inherently limited in their expressivity (e.g., what is the right representation of scooping onion pieces?), failing to capture nuanced features that may matter to the end-user (e.g., color plates).

% On the other hand, since in reality the robot operates on raw perceptual data like RGB images, visual representations obtained by powerful pre-trained vision models \citep{bla} promise to capture more nuanced features. However, key to making these useful for robotics is the training or tuning via proxy tasks  such as behavior cloning \citep{haldar2023watch, haldar2023teach} or temporal cycle-consistency learning \citep{dadashi2020primal}. \abnote{more proxy tasks??}

% If the robot sees video demonstrations of you cleaning your countertop, then it can use inverse reinforcement learning techniques \citep{bla}, to infer a reward signal that 
% that matter to \textit{you} all from raw perceptual inputs like RGB images is key. 
% State-of-the-art visual rewards automatically learn the visual representations from task specifications \citep{chen2021learning}, temporal progress \citep{zakka2022xirl, kumar2023graph}, a specified goal image \citep{ma2023vip}, or privileged access to action labels \citep{bla}. 


% \item To date, there has been tremendous progress in learning reward functions which capture human preferences \textit{assuming perfect state}
% Getting well-specified state-based features were traditionally hand-engineered \citep{ziebart2008maximum}, but  can also be learned interactively from human feedback \citep{bobu2021feature, katz2021preference} when the existing representation is not sufficient. 

% However, when the robot is deployed in reality, it does not have access to the true state of the world. 
% Of course, the robot can state estimation, but you don't even know what aspects of state is relevant to estimate.
% An alternative to this is for the robot to optimize a \textit{visual reward}, or a reward that takes as input raw observations, like RGB images, and outputs values that guide robot policy optimization. 
% This raises the question, what is the right visual reward that guides the robot's behavior to be aligned with the human's preferences?
% \item Although prior works considered hand-engineered representations of the visual input (e.g., distance to segmented regions \citep{kitani2012activity}), 

% \item This raises the question what is the visual reward that can help the robot do this? 
% \item If robots is to now optimize a reward from raw visual input, how can it learn a visual reward that captures the human's preferences?
% which break the traditional assumptions in human preference learning. 
% \item  The main reason these methods fail is because we no longer know the visual features. 
% \item If robots are to do this optimization from raw visual input, then the question is what is the visual reward that can help the robot do this? 
% \item This means that the ultimate judge of robot behavior is the human.
% \item However, human preferences go beyond temporal progress or goal-matching: for example, the preference of pushing food scraps in one group requires understanding that pick-and-place of each individual food scrap is an undesireable behavior.
% \item The problem is that we do not know the visual features that matter to the human a priori. 
% \item Thus, in this work, we argue that if a vision-based robot is to optimize for behaviors that are aligned with human preferences, the robot should understand the visual world the way that the human does. 

% induced by the robot's behavior match the \textit{human}'s preferences. 
% \abnote{alternative: what we really want is to have the \textit{visual features} induced by the robot's behavior match the visual features induced by the \textit{human} doing the task themselves.} 

% The preferences expressed in these videos are inherently personalized and go beyond goals: for example, cleaning a countertop includes both pushing food scraps into the trash can \textit{and} avoiding colliding with nearby bottles.




==> old_sections/intro_notes.tex <==
    % \item Vision-based robot learning has made tremendous progress in recent years: given a reward function, robot arms can learn manipulation skills \cite{kalashnikov2018qt, zeng2021transporter, shridhar2022cliport, haldar2023teach}, quadrupeds can gallop through complex terrain \cite{zhuang2023robot, agarwal2023legged}, and articulated hands can perform in-hand rotation \cite{akkaya2019solving, qi2023general}. 
    % and thus should behave in accordance with human preferences. 
    % \item For example, consider a robotic manipulator that is tasked with cleaning your kitchen countertop: there are food scraps that need to be tossed into the trash, and nearby bottles of oil and sauce. Your preferred way to clean up the countertop would be to push the food scraps all-at-once into the trash without knocking over any bottles.
    % \item However, before robots can generate \textit{how} to do the task, they needs to know \textit{what} about the task matters. For example, before the robot can clean a kitchen countertop, it needs to know what cleaning or orderly looks like
    % \item Vision-based robot learning has made tremendous progress in recent years, enabling robots to learn skills which optimize hand-engineered reward functions \cite{}. 
    % \item However, vision-based robot policies will not act in isolation; they will behave around and in service of humans. 
    % \item Here, visual rewards \cite{} have been key in guiding robot behavior during policy optimization, enabling the robot to \abnote{[insert why visual rewards are nice]}. 
    
% \textbf{Pitch-related thoughts.} Context: you have a pre-trained foundation model that understands the visual world, and you want to deploy it on a robot. The challenge: these models pay attention to "everything". Typically, figuring out what is relevant for a particular context is done through task or explicit reward signals. Instead, in this work, we argue that discovering what is relevant for a robot should be personalized and determined by the human end-user. In other words, we ask the question \textit{how can we learn human-centric visual representations for robotics?} 

% \textbf{Pitch Version 0:} Visual foundation models are powerful ways to build image- or video-based representations of the world, and offer promise for robots that act based on visual feedback.
% However, foundation models need to be fine-tuned for downstream robotics tasks.
% Typically, this robot-centric fine-tuning is done through self-supervised task signal (e.g., TCC) or engineered reward signals.
% However, if the robot using such a visual representation should be deployed around and in service of people, then these fine-tuning signals are not guaranteed to capture what matters to the ultimate end-user. In other words, the fine-tuned representations should be personalized for the human. 

% One idea is to fine-tune the robot’s visual representation from human feedback, like preference queries. This has been successful in crowd-sourced large language model alignment [cite].
% However, in the vision-based robotics domain there are two problems: (1) existing preference-based learning is very data inefficient to do for high-dimensional input data like image observations, and (2) SOTA human preference models assume that the person always gives feedback *in-distribution* of the robot embodiment [cite] -- for example, the robot shows the human a screen where the person selects a preferred behavior [cite]; or, the human teleoperates the robot to show what they like and don’t like [cite].

% In contrast, in real-world robotics settings, human feedback can come from more diverse sources of visual data -- a person can do the task on their own to show the robot what they like and what they don’t like. Or, the human can watch another human and express their preferences about the other human’s behavior. Or, the human can indicate which robot behaviors behaviors are aligned with their preferences.
% Inspired by this, our key idea is that human visual representations are *minimally embodiment-dependent*: human visual representations of a task are consistent regardless of if the human is doing the task themselves or if the robot is performing the task.
% If robots can take advantage of this, they can not only scalably fine-tune visual foundation models to be better aligned with human preferences, but they can also optimize for behaviors on their own embodiments which stay in distribution of the human preferences.

% In this work, we contribute:
% \begin{enumerate}
%     \item a unification of fine-tuning visual foundation models for robots
%     \item a new model for fine-tuning visual foundation models from human feedback which is minimally embodiment-dependent
%     \item quantitative experiments showing that our approach is both more data efficient and more robust to OOD data than prior RLHF models (e.g., direct reward prediction) and more aligned with human representations than self-supervised approaches (i.e., TCC).
% \end{enumerate}


\begin{itemize}
    % \item robots that operate on high-dimensional perceptual input like RGB images need to learn how to behave in accordance with human preferences. 
    % \item in the visual robotics domain, by far the most popular way is behavior cloning, which relies on labeled image-action pairs provided by the human to learn a robot policy. While promising, this is bad because this is very sensitive to domain shift and we need huge datasets of demonstrations for every task and every robot. Because you use actions, this also makes the embodiment of the agent super important (e.g., if the robot gets action labels). 
    % \item alternatively, we can try to learn a visual reward function which can be optimized by any robot. Crucial to this reward function is a \textit{representation} of the observations. Prior works have used TCC, MVP, but all
    % \item our idea is to come up with a visual reward that is aligned with the human's representation and incentivizes the robot to generate behaviors that stay in-distribution of the human's representation space. 
    % \item however, how do you know what features matter 
    % \item 
    \item Robots that operate on high-dimensional perceptual input like RGB images need to learn how to behave in accordance with human preferences. 
    \item Visual rewards are important to guide the robot behavior during policy optimization 
    \item Typically the visual rewards are matching the \textit{task} or the \textit{progress} or the \textit{goal} image.
    \item but, what we really want is to have the robot match the \textit{human}'s preference or the human's value. This is beyond notions like progress or goal-matching: e.g., instead of pushing carrots one-by-one, we prefer to group all the carrots together throughout the pushing. Or we prefer the coffee cup to stay away from our valuables like the computer. 
    \item In this work, we argue that if the robot is to optimize for behaviors that are aligned with human values, the robot should understand the visual world the way that the human does. 
    \item We extend the preference-based learning paradigm to the visual robot learning domain by developing a sample-efficient visual reward which captures what the human cares about. 
    \item By optimizing our novel visual reward, the robot is incentivized to stay in-distribution of the visual representation induced by the human teacher. 
    % \item However, we need a visual reward which encodes how the human sees the visual world and stays in-distribution of the representation induced by the 
    % \item To achieve this, our key idea is to 
    % interactively learn a visual representation from human preference feedback that only uses raw observations. and then leverage a visual reward function which encourages the robot to stay in-distribution 
    % \item we want robots to do behaviors in ways that humans like
    % \item if you have "privileged" access to action labels -- e.g., through robot teleoperation -- then life is good. You can match the human's preferred way of doing the task via various methods (e.g., LfD, IL, etc.)
    % \item However, in the real world we do not have actions because its a huge human cost to label actions 
    % \item as vision-based robot policies increasingly operate around and in service of humans, how can we ensure that these high-dim visual policies are aligned with human preferences? 
    % % \item robots will take actions around humans only using raw perceptual input
    % % \item the question is, how can these high-dim visual policies optimize for behaviors that are aligned with the human's preferences? 
    % \item by far the most popular way is to rely on action labels provided by the human to do behavior cloning. This is bad because we need huge datasets of demonstrations for every dataset and every robot. Because you use actions, this makes the embodiment of the agent super important (e.g., if the robot gets action labels). 
    % \item an alternative approach is to learn a reward function which can be optimized by \textit{any} robot. 
    
    % naievly applying this to the visual domain suffers from spurrious correlations and low sample efficiency. 
    % \item alternatively, you can come up with a visual reward which can be optimized by \textit{any} robot. 
    % \item However, this reward function needs to somehow stay in-distribution of the human's preferred behavior. 
    % \item this requires two things: 1) a way to match the behavior and 2) 
    % \item prior works use MVP or TCC to build a visual representation 
    % \item 
    % \item 
    
    % \item 
    % \item in state-space, you can do this via feature matching in IRL or via imitation learning 
    % \item however, if you aren't in state space, and if you are 
    % \item but you 

    % \item when robots are deployed in service of people, they need to perform tasks in ways that humans prefer. 
    % \item this is challenging, because the robot does not know the correct objective function to optimize a priori. This is further complicated because how the human prefers the task done is based on their visual representation, or how they interpret the visual world. 
    % \item Our key idea is the robot's visual reward should incentivize behaviors that are in-distribution of the human's internal representation of the visual world. 
    % \item 
    % \item This raises two natural challenges: 1) in-distribution and 2) preferred representation. 
\end{itemize}



\textbf{Pitch Version 2:}
\begin{itemize}
    \item when robots are deployed around and in service of people, they need to use perceptual sensors like RGB cameras to understand what visual features of the task matter to the end-user. 
    \item For example, consider a robotic manipulator that is tasked with cleaning your kitchen countertop: there are chopped up pieces of onion and carrot, food scraps that need to be tossed into the trash, and nearby bottles of oil and sauce. Your preferred way to clean up the countertop would be to push the food scraps all-at-once into the trash without knocking over any bottles, and rearrange the onion and carrot pieces to be grouped together without touching or mixing. 
    \item In contrast, an \textit{undesirable} way to clean up the countertop involves objects colliding during rearrangement, being manipulated inefficiently (e.g., each scrap is pushed into the trash one-by-one), and the food pieces mixing.
    \item on one hand, the robot could infer the human's preferences by mapping visual observations to a scalar reward. In non-vision-based robotics domains [cite] or in the LLM domain [cite], this is typically done via preference-based learning: the human ranks robot behavior as more or less desirable and the robot infers the associated reward. This is nice because by using human feedback, the robot can hopefully learn the human’s preferred way of doing the task and \textit{implicitly} learn the human's visual features. However, directly learning this mapping from high-dimensional input space like images is (1) data inefficient [cite]and (2) prone to spurious correlations in the implicitly learned representation [cite].
    % \item on the other hand, the robot could focus \textit{explicitly} on learning a visual representation of the task that matches with the visual features that the human cares about. Existing methods for doing this by fine-tuning pre-trained visual representations [cite] task-relevant signals. For example, they assume that the end-user is an expert and can generate expert actions on the robot’s embodiment [cite], or they assume that the robot already knows a good reward function with which it tunes its visual representation of the task [cite]. However, in reality neither of these two visual representation learning methods are realistic for personal robotics: end-users aren't expert teleoperators [cite], and if the robot already knew the right reward that mattered to the end-user, then it could just optimize for it.
    \item in this work, we propose a method to get the best of both worlds: use human feedback to learn the user’s preferred visual representation, and then use this preference-aligned representation for robot behavior generation
    \item specifically, our method utilizes few (i.e., $\leq 30$) video demonstrations of an end-user performing a task in ways consistent with their preferences that are ranked in order of desirability. The preferences expressed in these videos are inherently personalized and go beyond goals: for example, cleaning a countertop includes both pushing food scraps into the trash can \textit{and} avoiding colliding with nearby bottles. Using this insight, we formulate a metric learning problem to infer visual features which disambiguate the preferred and less-preferred human video demonstrations.
    \item using this personalized visual representation, we then enable the robot to optimize behaviors that are consistent with the human’s task preference. Specifically, we take inspiration from optimal transport to design a dense, embodiment-agnostic reward signal that measures the representation alignment between videos induced by the robot and the videos of the end-user used during representation learning.
\end{itemize}



==> old_sections/method.tex <==
% \section{Visual Representation Alignment}
\section{RAPL: Representation-Aligned Preference-Based Learning}

% \begin{itemize}
%     % \item Our key idea is that if the robot's behavior is aligned with the human's preferences, then it will induce a similar distribution in the human's visual representation space to that of the human's policy. In other words, the empirical distribution $P(\reph(\obstraj) \mid \policyr)$ will be ``close'' to the empirical distribution of $P(\reph(\obstraj) \mid \policyh)$. 
%     % \item However, before we can measure how close these distributions are, the question of \textit{which} embedding remains, since we do not know $\reph$. 
%     % \item  We can leverage advances in optimal transport \citep{bla} to measure the distance between these embedding distributions, but the question of \textit{which} embedding remains, since we do not know $\reph$. 
%     % \item Crucial to the optimal transport based reward function is the representation model $\phi$ that maps a raw image to a latent embedding. 
%     % \item Previous works have attempted to learn such an encoder through behavior cloning \citep{haldar2023teach} or using off-the-shelf encoders pretrained on large-scale datasets \citep{deng2009imagenet, xiao2022masked, nair2022r3m, radosavovic2023real}. On the one hand, learning the representation model with behavior cloning as the proxy task requires actions labels which are often not available. On the other hand, pre-trained visual representation models using unsupervised or self-supervised learning methods are prone to learn representations that can not disambiguate between what  ``matters'' to the task versus what is spurious, leading to misaligned robot behavior.
%     \item In this work, we propose that robots should leverage human feedback---specifically preference queries---to align their visual representations with the end user (i.e., bring $\repr$ and $\reph$ closer together). 
%     % \item We advocate that robot's representations should encode information that are not only functional but also what humans care about so the visual reward incentivizes the robot to so what humans prefer. To this end, we aim to \textit{align} the robot's representation model with human preferences and values. In this section, we formalize the representation alignment problem and provide an approximation solution.
%     \item We first formalize this visual representation alignment problem and then provide an approximate solution through the lens of preference-based learning and optimal transport.
%     % \item In this work, we want to understand how the robot can optimize behaviors that are preferred under the human's visual representation $\reph$.
% \end{itemize}


% First, using pre-trained visual models has become an increasingly popular way to design $\repr$, where the representation is fine-tuned through proxy tasks like dynamics prediction \citep{}, action prediction \citep{}, or temporal cycle consistency \citep{zakka2022xirl, kumar2023graph}. 
% However, these all bypass the human’s input on what matters to \textit{them}.
In this work, we leverage pre-trained visual encoders but advocate that robots fine-tune them with \textit{preference-based human feedback} to extract visual features that are relevant for how the end-user likes the task to be performed. 
% , while
% to align them with human preferences. 
% to preserving those that are hard to hand-engineer. 
% leverage pre-trained visual models capable of modeling nuanced features that are hard to hand-encode, 
% i feel like there is a lot of "preferences here"...
% (i.e., bring $\repr$ and $\reph$ closer together). 
Preference-based feedback, where a user is asked to compare two or more trajectories, has been shown to be easier for end-users to provide compared to direct labelling or giving near-optimal demonstrations \citep{wirth2017survey}. 
% and has been successful in the natural language domain, state-space robotics domain, and AI more broadly \citep{}. 
However, we are the first to use preference-based human feedback to align pre-trained visual models with user preference for robot learning.

Once the robot has an aligned representation, what reward should it optimize to generate preferred behaviors?
% \tr{why this answer's the first question? I feel there is a logic jump here...} \abnote{agreed; do you have a better intro sentence suggestion?}
% Since the human's preference feedback is generated from their policy $\policyh$, then we know it also leaks information about their true reward $\rewh$. 
% for realistic learning from end-users.
% This sample inefficiency is prohibitive for real-world learning from end-users.
To reduce the sample complexity, we use optimal transport methods to design a visual reward  \citep{villani2009optimal}, and focus the preference feedback exclusively on fine-tuning the representation. 
Since optimal transport methods are a way to optimize Integral Probability Metrics in a principled manner, the transport plan exactly yields a reward which maximizes feature matching between the learner and the expert \textit{in our aligned representation space}.
% in a principled manner. 
% provides a principled, dense signal during policy optimization, incentivizing the robot to stay in-distribution of the aligned visual representation induced by the human teacher.
% If the robot’s behavior is aligned with the human’s preferences, then it will induce a similar distribution in the human’s visual representation space to that of the human’s policy.

In this section, we first formally state the visual representation alignment problem by drawing upon recent work in cognitive science \citep{sucholutsky2023alignment} and then detail our approximate solution, \textbf{R}epresentation-\textbf{A}ligned \textbf{P}reference-based \textbf{L}earning (\textbf{RAPL}), through the lens of preference-based learning and optimal transport. In addition to this section's content, we also provide more details about comparisons between our work and previous work in Appendix~\ref{app:related_work} and~\ref{app:questions}.

\subsection{The Visual Representation Alignment Problem for Robotics}
\label{subsec:rapl_formalism}

% Following prior works \citep{jamieson2011low, sucholutsky2023alignment} that leverage non-metric similarity triplets to recover hidden psychological representations, we propose a triplet-based definition of representation alignment problem.

We follow the formulation in \cite{sucholutsky2023alignment} and bring this to the robot learning domain. Intuitively, visual representation alignment is defined as the degree to which the output of the robot's encoder, $\repr$, matches the human's internal representation, $\reph$, for the same image observation, $
\obs \in \mathcal{O}$, during task execution.
%\textit{conditioned on the task (e.g., clean counter-top) and human's preferences (e.g., stack plates based on color)}. 
% Intuitively, if the robot understands the visual features that matter to the person, then it's visual representation is able to produce similar features. 
We utilize a triplet-based definition of representation alignment as in \citep{ jamieson2011low} and \citep{sucholutsky2023alignment}.


% Below, we formalize this mathematically. 
    
\begin{definition}[Triplet-based Representation Space] Let $\obstraj = \{\obs^t\}^T_{t=0}$ be a sequence of image observations over $T$ timesteps, $\phi : \mathcal{O} \rightarrow \Phi$ be a given representation model, and $\phi_{}(\obstraj) := \{\phi(\obs^{0}),\dots,\phi(\obs^{T})\}$ be the corresponding embedding trajectory. For some distance metric $d(\cdot, \cdot)$ and two observation trajectories $\obstraj^{i}$ and $\obstraj^{j}$, let $d\big(\phi_{}(\obstraj^{i}),\phi_{}(\obstraj^{j})\big)$ be the distance between their embedding trajectories. The triplet-based representation space of $\phi$ is:
\begin{equation}
\begin{aligned}
S_{\phi_{}} = \Big\{(\obstraj^{i},\obstraj^{j},\obstraj^{k}) : d\big(\phi_{}(\obstraj^{i}),\phi_{}(\obstraj^{j})\big) < d\big(\phi_{}(\obstraj^{i}),\phi_{}(\obstraj^{k})\big), \obstraj^{i,j,k} \in \Xi \Big\},
\end{aligned}
\label{eq:representation_space}
\end{equation}
where $\Xi$ is the set of all possible image trajectories for the task of interest.
\end{definition}

%Crucial to the above definition is distance $d$ that defines the similarity between observation trajectories.


%In theory, this distance should be the reward, but however we do not. In our setting, we precisely do not know how to judge which of these are 
%An approximately rational human would use their $\rewh$ which encodes their task preferences to assess this distance. However, we do not have direct access to this function $d(\cdot, \cdot)$. d is like relative reward instead of absolute reward.  


%\abnote{technically $\phi$ operates on individual images, not on the image trajectory...}
Intuitively, this states that the visual representation $\phi$ helps the agent determine how similar two videos are in a lower-dimensional space. For all possible triplets of videos that the agent could see, it can determine which videos are more similar and which videos are less similar using its embedding space. The set $S_{\phi}$ contains all such similarity triplets. 

%\abnote{I feel there is a confound between "similar" and "preferred" here. In vanilla PBRL, we say that $\xi_A \succ \xi_B$ if $\xi_A$ has greater reward than $\xi_B$. Can we connect to this?}
% $d\big(\phi_{}(\obstraj^{i}),\phi_{}(\obstraj^{j})\big) < d\big(\phi_{}(\obstraj^{i}),\phi_{}(\obstraj^{k})\big)$ encodes the similarity comparison under representation model $\phi$: $\obstraj^i$ is closer to $\obstraj^j$ compared to $\obstraj^k$.

\begin{definition}[Visual Representation Alignment Problem]
Recall that $\reph$ and $\repr$ are the human and robot's visual representations respectively. The representation alignment problem is defined as learning a $\repr$ which minimizes the difference between the two agents' representation spaces, as measured by a function $\ell$ which penalizes divergence between the two representation spaces:
\begin{equation}
\begin{aligned}
\min_{\phi_{\mathrm{R}}} \ell(S_{\phi_{\mathrm{R}}}, S_{\phi_{\mathrm{H}}}).
\end{aligned}
\label{eq:representation_alignment_problem}
\end{equation}
\end{definition} 



\subsection{Representation Inference via Preference-based Learning}
\label{subsec:rapl_inference}
% Approximate Representation Alignment via Preference-based Learning
% Aligning Robot and Human Representations

Although this formulation sheds light on the underlying problem, solving \autoref{eq:representation_alignment_problem} exactly is impossible since the functional form of the human's representation $\phi_{\mathrm{H}}$ is unavailable and the set $S_{\phi_{\mathrm{H}}}$ is infinite. Thus, we approximate the problem by constructing  a subset $\tilde{S}_{\reph} \subset S_{\reph}$ of triplet queries. 
Since we seek a representation that is relevant to the human's preferences, we ask the human to rank these triplets based on their \textit{preference-based} notion of similarity (e.g., $\rewh(\reph(\obstraj^i)) > \rewh(\reph(\obstraj^j)) > \rewh(\reph(\obstraj^k)) \implies \obstraj^i \succ \obstraj^j \succ \obstraj^k$). With these rankings, we implicitly learn $\reph$ via a neural network trained on these triplets.

% \begin{definition}[Preference-Based Similarity]
% Since our ultimate goal is to align robot behavior with human preference, we define similarity as how close in
% preference-space the observations are, i.e., $\obstraj^j$ is similar to $\obstraj^i$ compared to $\obstraj^k$ because $\obstraj^i$ and  $\obstraj^j$ have similar rewards compared to $\obstraj^j$. Or sth like we ask the user to use their preference to do this ranking..
% \end{definition}


We interpret a human’s preference over the triplet $(\obstraj^{i},\obstraj^{j},\obstraj^{k}) \in \tilde{S}_{\reph}$ via the Bradley-Terry model \citep{bradley1952rank}, where $\obstraj^{i}$ is treated as an anchor and $\obstraj^{j}, \obstraj^{k}$ are compared to the anchor in terms of similarity as in \autoref{eq:representation_space}:
\begin{equation}
\begin{aligned}
\mathbb{P}(\obstraj^i \succ \obstraj^j \succ \obstraj^k \mid \reph) \approx \frac{e^{-d(\reph(\obstraj^i), ~\reph(\obstraj^j))}}{e^{-d(\reph(\obstraj^i), ~\reph(\obstraj^j))} + e^{-d(\reph(\obstraj^i), ~\reph(\obstraj^k))}}.
\end{aligned}
\label{eq:representation_alignment_loss}
\end{equation}
A natural idea would be to leverage the human's preference feedback to do direct reward prediction (i.e., model both $d$ and $\reph$ via a single neural network to approximate $\rewh$), as is done in traditional preference-based reward learning \citep{christiano2017deep}.
However, we find empirically (Section~\ref{subsec:in-domain-manipulation}) that directly learning a high-quality visual reward from preference queries requires a prohibitive amount of human feedback that is unrealistic to expect from end-users \citep{brown2019extrapolating, bobu2023aligning}. 


Instead, we focus all the preference feedback on just representation alignment. But, this raises the question what distance measure $d$ should we use?
In this work, we use optimal transport as a principled way to measure the feature matching between any two videos. 
% and then utilize the optimal transport plan as $d(\cdot, \cdot)$ which provides a principled way to measure distance between embedding distributions.
% penalizes the coupling between the embedding distribution of the preferred and less-preferred visual demonstrations (more details in Section~\ref{subsec:rapl_visual_reward} and Appendix~\ref{app:OT}). 
% We choose the distance function $d(\cdot, \cdot)$ to be the entropy regularized Wasserstien distance between the two latent distributions:
% \begin{align}
%     d(\reph(\obstraj^i), \reph(\obstraj^k)) = \sum_{t=1}^{T}\sum_{\tau=1}^{T} c\big(\reph(o^{i,t}), \reph(o^{k,\tau})\big)\mu^{*}_{t,\tau}.
% \end{align}
% \abnote{maybe we allude to this but don't mathematically define it here, and say that the mathematical details are presented in the next section?} 
% let $\mathcal{D}_+ \subset \mathcal{S}_{\reph}$ be a dataset of preferred videos from the preference video dataset and $\mathcal{D}_\robot$ be the set of videos induced by a given robot policy $\policyr$. 
For any video $\obstraj$ and for a given representation $\phi$, let the induced empirical embedding distribution be $\rho = \frac{1}{T} \sum_{t=0}^{T} \delta_{\phi(\obs^t)}$, where $\delta_{\phi(\obs^t)}$ is a Dirac distribution centered on $\phi(\obs^t)$. 
Optimal transport finds the optimal coupling $\mu^* \in \mathbb{R}^{T \times T}$ that transports one embedding distribution, $\rho_i$, to another video embedding distribution, $\rho_j$, with minimal cost. This approach has a well-developed suite of numerical solution techniques \citep{peyre2019computational} which we leverage in practice (for details on this see App.~\ref{app:OT}).



Our final optimization is a maximum likelihood estimation problem:
\begin{align}
    \approxreph := \max_{\reph} \sum_{(\obstraj^{i},\obstraj^{j},\obstraj^{k})\in\tilde{S}_{\reph}} \mathbb{P}(\obstraj^i \succ \obstraj^j \succ \obstraj^k \mid \reph).
    \label{eq:representation_optimization}
\end{align}
Since the robot seeks a visual representation that is aligned with the human's, we set: 
\begin{equation}
    \repr := \approxreph.
\end{equation}


% \textbf{Design Details.} \abnote{Put here the structure of the neural network, how you construct this set $\tilde{S}_{\reph}$, what optimizer you used to solve \autoref{eq:representation_optimization}.}\tr{Lets's put this in the experiment setting?} \abnote{we could put here any details that are uniform across all experiments?}\tr{The reason that I want to put it the result section is because I don't want to give readers the impression that it only works in resnet. The method could be applied to any backbone.}

% \max_{\phi_{\mathrm{R}}} \sum_{(\xi^{i},\xi^{j},\xi^{k})\in\Tilde{S}_{\phi_{\mathrm{H}}}} 

%Then we can learn $g$ with differentiable Sinkorn algorithm \cite{Gould:PAMI2022} 

\subsection{Preference-Aligned Robot Behavior via Optimal Transport}
\label{subsec:rapl_visual_reward}
% \subsection{A Sample-Efficient Visual Reward via Optimal Transport}

% We leverage optimal transport during both representation learning from human feedback and during robot policy optimization. 
Given our aligned visual representation, we seek a robot policy $\policyr$ whose behavior respects the end-user's preferences. 
%Unfortunately, in our setting the robot does not have access to the action labels associated with the video demonstrations in $\tilde{S}_{\reph}$, making behavior cloning methods infeasible. 
% On the other hand, directly doing Inverse Reinforcement Learning (IRL) \citep{abbeel2004apprenticeship, ziebart2008maximum} where the robot predicts (and then optimizes) rewards from image observations requires numerous near-optimal demonstrations \citep{bla}. 
%On the other hand, 
Traditional IRL methods \citep{abbeel2004apprenticeship, ziebart2008maximum} are built upon matching features between the expert and the learner. Leveraging this insight, we use optimal transport methods since the optimal transport plan is equivalent to defining a reward function that encourages this matching \citep{kantorovich1958space}.
% and this approach is associated with a suite of numerical techniques \citep{peyre2019computational}. %matches the embedded state visitation frequency. 

% To circumvent these issues, we take inspiration from recent works that leverage optimal transport theory \citep{villani2009optimal} to compute reward functions directly in high-dimensional visual spaces \citep{haldar2023watch, haldar2023teach}. 
% We investigate this approach in our setting to generate a visual reward signal from raw video observations. 
% One of its key advantages is that it provides an intuitive but dense signal on the distance between two distributions, as measured via the optimal transport of probability mass from one distribution to the other. 
% One of its key advantages is that it provides a principled way to compare occupancy measures between two agent's policies even in high-dimensional spaces. 
% The distance between these two distributions is measured via the optimal transport of probability mass from one distribution to the other.  
% \textbf{Setup.} Let $\mathcal{D}_+ \subset \mathcal{S}_{\reph}$ be a dataset of preferred videos from the preference video dataset and $\mathcal{D}_\robot$ be the set of videos induced by a given robot policy $\policyr$. 
% For any video $\obstraj$, let the induced empirical embedding distribution be $\rho = \frac{1}{T} \sum_{t=0}^{T} \delta_{\repr(\obs^t)}$, where $\delta_{\repr(\obs^t)}$ is a Dirac distribution centered on $\repr(\obs^t)$. 

% For a video $\obstraj_+ \in \mathcal{D}_+$, let $\rho_+$ be its empirical embedding distribution, and for $\obstraj_R \in \mathcal{D}_\robot$ let $\rho_\robot$ be the corresponding embedding distribution. 

% \textbf{Visual Reward.} 
% by solving the optimization problem that minimizes the Wasserstin distance between two distributions. 
%     \begin{equation}
%     \begin{aligned}
%     \mu^{*} = \argmin_{\mu \in \mathcal{M}(\rho_{\mathrm{R}}, \rho_{e})} \sum_{t=1}^{T}\sum_{t'=1}^{T} c\big(\phi(o^t_e), \phi(o^t_{\mathrm{R}})\big)\mu_{t,t'},
%     \end{aligned}
%     \label{eq:ot_problem}
%     \end{equation}
% where $\mathcal{M}(\rho_{\mathrm{R}}, \rho_{e}) = \{\mu \in \mathbb{R}^{T \times T}: \mu\mathbf{1} = \rho_{\mathrm{R}}, \mu^{T}\mathbf{1} = \rho_e\}$ is the set of coupling matrices and $c: \mathbb{R}^{n_e} \times \mathbb{R}^{n_e}\rightarrow \mathbb{R}$ is a cost function defined in the embedding space (e.g., cosine distance). 

Specifically, we seek to match the \textit{embedded} observation occupancy measure induced by the robot's policy $\policyr$, and the embedded observation occupancy measure of a human's preferred video demonstration, $\obstraj_+$. Thus, the optimal transport plan yields the reward which is optimized in \autoref{eq:robot_planning_problem}:
\begin{equation}
\begin{aligned}
\rewr(\obs^t_\mathrm{R}; \repr) = -\sum_{t'=1}^{T} c\big(\repr(\obs^{t}_\robot), \repr(\obs^{t'}_+)\big)\mu^{*}_{t, t'},
\end{aligned}
\label{eq:ot_reward}
\end{equation}
where $\mu^{*}$ is the optimal coupling between the empirical embedding distributions induced by the robot and the expert.
% and the expert demonstration's embedding distribution.
% that incentivizes the robot to align its observation distribution with the expert's distribution.
% The reward function incentivizes the robot to stay within the expert demonstration distribution by explicitly minimizing the distance between the observation distribution and expert distribution. 
This reward has been successful in prior vision-based robot learning \citep{haldar2023teach, haldar2023watch, guzey2023see} with the key difference in our setting being that we use RAPL's aligned visual representation $\repr$ for feature matching (for details on the difference between our approach and prior OT based visual reward see Appendix~\ref{app:questions}). 
% During reinforcement learning, this reward incentivizes the robot to stay in-distribution of the preferred video's visual features obtained via RAPL's representation, $\repr$. 
% See more details in App.~\ref{app:OT}. 

    
% Solving the above optimisation (\ref{eq:ot_problem}) directly is generally intractable for high dimensional distributions. In practice, we solve a entropy regularized version of the problem following the Sinkhorn algorithm \cite{peyre2019computational}:
% \begin{equation}
%     \begin{aligned}
%     \mu^{*} = \argmin_{\mu \in \mathcal{M}(\rho_{\mathrm{R}}, \rho_{e})} \sum_{t=1}^{T}\sum_{t'=1}^{T} c\big(\phi(o^t_e), \phi(o^t_{\mathrm{R}})\big)\mu_{t,t'} - \epsilon\mathcal{H}(\mu),
%     \end{aligned}
% \label{eq:ot_problem_regu}
% \end{equation}
% where $\mathcal{H}$ denotes the entropy term that regularizes the optimization and $\epsilon$ is the associated weight. 





% \textbf{Design Details.} \abnote{Describe relevant details like how the robot's policy is a neural network, how you optimize the robot policy via PPO, what optimizer you use, what simulator you use, etc. }
% \tr{Lets's put this in the experiment setting?}

==> old_sections/releated_work.tex <==

\subsection{Motivating questions}
\label{app:questions}

Inspired by the appendix of \citep{karamcheti2023language}, in this section, we list some motivating questions that may arise from reading the main paper.


\textit{\textbf{Q1.} The experiments all consider preferences beyond task progress. If the end-user's preference is only progress, can RAPL achieve comparable performance compared to the SOTA TCC-based visual reward \citep{zakka2022xirl}?}

\begin{wrapfigure}{r}{0.4\textwidth}
    \vspace{-0.5cm} \includegraphics[width=0.4\textwidth]{figs/xirl_ot_exp.pdf}
    \vspace{-0.8cm}
    \caption{\textbf{X-Magical.} Progress-only reward success rate.}
    \label{fig:tcc_vs_rapl}
    \vspace{-0.2cm}
\end{wrapfigure}

To investigate this, we return to the X-Magical \textbf{grouping} task (middle plots in Figure~\ref{fig:x-magical-env}) where a short stick robot needs to push two objects to goal. 
We removed the grouping preference so the ground truth task reward is consistent with the original benchmark in \citep{zakka2022xirl}. 
We trained RAPL with $150$ preference queries and compare it with the TCC reward model trained using $500$ demonstrations. 
In Figure~\ref{fig:tcc_vs_rapl}, we show the policy evaluation success rate during policy learning. 
We see that \rapl has comparable final success rate compared to \tcc and has a more stable policy training, showing that it can learn a superset of preferences when compared to TCC.


\textit{\textbf{Q2.} What makes RAPL different from prior robot learning works that use optimal transport (OT) based visual rewards?}

Indeed, OT-based visual rewards have become increasingly popular for learning robot manipulation \citep{haldar2023teach, haldar2023watch, guzey2023see}. However, key to making the OT-based visual reward successful in  \cite{haldar2023teach} is fine-tuning the representation model via behavior cloning tasks. This helps the model to capture some task-relevant information at the cost of requiring action labels. Furthermore, by relying on action labels, it is unclear if the learned reward can generalize to a different embodiment. 
Instead, our approach learns the representation only using preference queries (no action labels) and can generalize to embodiments.

% \textit{\textbf{Q3.} What makes RAPL different from prior representation alignment for reward learning works?}
% \tr{To do: compare with SIRL}

\textit{\textbf{Q3.} Why do \mvpot and \tccot achieve near 0 success rate in the robot manipulation experiments in Figure~\ref{fig:franka_success_v_reward} and Figure~\ref{fig:kuka_success_v_reward}?}

Recall that both \mvpot and \tccot use optimal transport to match the embedding distribution of the robot and the expert, but they vary which visual representation they use to obtain the embedding.
% visual rewards incentivize the robot to match the visual representation distribution induced by expert demonstration, but vary the image encoder. 

The MVP encoder is trained via masked autoencoding \citep{he2022masked} to reconstruct heavily masked video frames. As such, it captures representations amenable to per-pixel reconstruction. Prior work \citep{karamcheti2023language} has demonstrated that this representation struggles with higher-level problems (e.g., language-based imitation). We hypothesize this is why \mvpot struggles to capture preference-relevant features and does not lead to aligned robot behaviors.
% captures representations that are tailored for image reconstruction, thus matching such a representation distribution does not lead to behavior level matching. 
Our results are also consistent with the experiments in \citep{haldar2023teach} where an OT-based visual reward with a pre-trained MVP representation model gives near 0 success rate for manipulation tasks.

The TCC encoder is trained via temporal cycle-consistency constraints, and as such captures representations that encode solely task progress (e.g., distance to the goal image). 
Such a representation works well when goal reaching is the only preference of the end user. In our tabletop grouping task, the end user cares about goal reaching, but they also prefer moving the two objects together to goal region over moving the objects one-by-one. Thus if the robot happens to push one object towards the goal during policy learning, \tccot will reward this behavior (since this image is getting ``closer'' to the goal image) even though this is not preferred by the user.  
 


\subsection{Extended Related Work}
\label{app:related_work}
% \textbf{Visual representations for robotic learning.}
% Unsupervised/self-supervised R3M \cite{nair2022r3m}, Voltron \cite{karamcheti2023language}, Cortex\cite{majumdar2023we}, MVP \cite{radosavovic2023real}
% Our work draws upon advances in several domains from visual reward learning, preference-based learning, and optimal transport. Here we summarize the relevant literature. 

\textbf{Visual robot rewards}
% are an increasingly popular way of solving the inverse reinforcement learning (IRL) problem directly from video observations.  
promise to capture task preferences directly from videos. 
Self-supervised approaches leverage task progress inherent in video demonstrations to learn how ``far'' the robot is from completing the task \citep{zakka2022xirl, kumar2023graph, ma2023vip} 
while other approaches identify task segments and measure distance to these subgoals \citep{sermanet2016unsupervised, tanwani2020motion2vec, shao2020concept, chen2021learning}. 
However, these approaches fail to model preferences \textit{during} task execution that go beyond progress (e.g., spatial regions to avoid during movement). 
Fundamental work in IRL uses feature matching between the expert and the learner in terms of the expected state visitation distribution to infer rewards \citep{abbeel2004apprenticeship, ziebart2008maximum}, and recent work in optimal transport has shown how to scale this matching to high dimensional state spaces \citep{xiao2019wasserstein, dadashi2020primal, papagiannis2022imitation, luo2023optimal}. 
However, key to making this matching work from high-dimensional visual input spaces is a good visual embedding. 
Previous works used proxy tasks, such as behavior cloning \citep{haldar2023watch, haldar2023teach} or temporal cycle-consistency learning \citep{dadashi2020primal}, to train the robot's visual representation. 
In contrast to prior works that rely on hard-to-obtain action labels or using only self-supervised signal, we propose an OT-based visual reward that is trained 
purely on videos (no action labels needed) that ranked by the \textit{end-user's} preferences. 
% However, these tasks either require direct action labels that are hard to obtain, or bypass the human’s input on what matters to them, exacerbating spurious correlations and ultimately leading to misaligned robot behaviors. 
% Different from previous works, our OT-based visual reward is trained purely based on videos with representations that are aligned with human preference, yielding robot behavior that aligned with the end-user's preference and further unlocking efficient cross-embodiment learning.



%\abnote{this is just copied over from a different section}
%Previous works have attempted to fine-tune representations in pre-trained visual models through behavior cloning \citep{haldar2023teach} or using off-the-shelf encoders pretrained on large-scale datasets \citep{deng2009imagenet, xiao2022masked, nair2022r3m, radosavovic2023real}.
%On the one hand, learning the representation model with behavior cloning as the proxy task requires actions labels which are often not available. On the other hand, pre-trained visual representation models using unsupervised or self-supervised learning methods are prone to learn representations that can not disambiguate between what ``matters'' to the task versus what is spurious, leading to misaligned robot behavior.

\textbf{Preference-based learning.} 
While demonstrations have been the data of choice for reward learning in the past, an increasingly popular approach is to use preference-based learning \citep{christiano2017deep, sadigh2017active, biyik2018batch, wirth2017survey, brown2019extrapolating, stiennon2020learning, zhang2022time, shin2023benchmarks}. Here the human is asked to compare two (or more) trajectories (or states), and then the robot infers a map from ranked trajectories to a scalar reward. This feedback is often easier for people to give than kinesthetic teaching or fine-grained feedback \citep{shin2023benchmarks}.
% In robotics settings where the low-dimensional state and features are well-specified and carefully hand-crafted \citep{sadigh2017active, biyik2018batch}, this approach has been successful.
At the same time, prior works and our experiments show that directly predicting the reward from preference queries and high-dimensional input suffers from high sample inefficiency and causal confusion \citep{bobu2023aligning, tien2022causal}. 
% However, both previous works \citep{bobu2023aligning} and our experiments show that directly predicting the reward from high dimensional input suffers from sample inefficiency, especially when human needs to provide such feedback, and poor generalization. 
To mitigate this issue, \citep{brown2020safe} augments multiple self-supervised objectives like inverse dynamics prediction or enforcing temporal cycle-consistency with the preference learning loss, but this requires additional signals like actions and the additional self-supervised objective may bias the learned rewards towards capturing spurious correlations.

% \textbf{Reward \& Representation Learning in State Space.} If the robot has access to the true state of the world, then there are a large suite of techniques for learning reward functions which capture human preferences [cite]. These approaches have shown that if the reward function has well-specified \textit{state-based features} then the true human's reward can be recovered \citep{ziebart2008maximum, levine2011nonlinear, finn2016guided, biyik2020active}. However, when the features are incomplete \citep{bobu2020quantifying}, or contain spurious correlations \citep{tien2022causal}, then preference learning suffers, and methods like interactive feature augmentation are needed \citep{bobu2021feature, katz2021preference}. 

\textbf{Representation alignment in robot learning.} Representation alignment studies the agreement between the representations of two learning agents.
%Aligning AI systems' representation with human's has been long studied in cognitive science, image classification tasks \citep{nanda2021exploring, fel2022harmonizing, sucholutsky2023alignment}
As robots will ultimately operate in service of people, representation alignment is becoming increasingly important for robots to interpret the world in the same way as we do.
Previous work has leveraged user feedback, such as human-driven feature selection \citep{bullard2018human, luu2019incremental}, interactive feature construction \citep{bobu2021feature, katz2021preference}, or similarity-implicit representation learning \citep{bobu2023sirl}, to learn aligned representations for robot behavior learning. But they either operate on a manually defined feature set or learning features in low-dimensional state space settings (e.g., positions).
In the visual domain,
\citep{zhang2020learning} uses a per-image reward signal to align the image representation with the preferences encoded in the reward signal; however, when the main objective is learning the human's reward then assuming a priori access to such a reward signal is not feasible. 
Instead, our work utilizes human preference feedback to align the robot's visual representations with the end user and optimal transport as our embedding-based reward function.


%\citep{tanwani2020motion2vec} Use behavior classification loss to learn representations that can be used to classify the action type of a demonstration.

%\citep{nanda2021exploring} alignment in the image classification domain, not in the video / behavior domain. 

% \textbf{Optimal transport based rewards.}

==> old_sections/setup.tex <==
\section{Problem Setup}

\textbf{Human Policy.} 
We consider scenarios where the robot R wants to learn how to perform a task for human H. 
The human knows the desired reward $\rewh$ which encodes their preferences for the task. The human acts via an approximately optimal policy $\policyh^{*}: \mathcal{O} \rightarrow \mathcal{U}_\human$ based on their underlying reward function. 
Instead of directly consuming the raw perceptual input, research suggests that humans naturally build visual representations of the world \citep{bonnen2021ventral} that focus on task-relevant attributes \citep{callaway2021fixation}. 
We model the human's representation model as $\reph: \mathcal{O} \rightarrow \Phi_{\mathrm{H}}$, mapping from the perceptual input $o \in \mathcal{O}$ to the human's latent space $\Phi_{\mathrm{H}}$ which captures their task and preference-relevant features.

\textbf{Robot Policy.} We seek to learn a robot policy $\policyr^*: \mathcal{O} \rightarrow \mathcal{U}_\robot$ which maps from image observations to actions that maximizes a reward: 
\begin{equation}
\begin{aligned}
\policyr^* = \arg\max_{\policyr}  \mathbb{E}_{\obstraj \sim p(\obstraj \mid \policyr)} \Big[ \sum_{t=0}^{\infty} \gamma^t \cdot \rewr(\repr(\obs^t))\Big],
\end{aligned}
\label{eq:robot_planning_problem}
\end{equation}
where $\gamma \in [0,1)$ is the discount factor and $\obstraj = \{\obs^0, \obs^1, \hdots \}$ is the image observation trajectory induced by the robot's policy. 
The robot's reward $\rewr$ relies on a visual representation, $\repr: \mathcal{O} \rightarrow \Phi_\robot$, which maps from the image observation $\obs \in \mathcal{O}$ to a lower-dimensional latent space, $\Phi_\robot$. In general, this could be hand-crafted, such as distances to objects from the agent's end-effector \citep{ziebart2008maximum, levine2011nonlinear, finn2016guided}, or the output of an encoder pre-trained on large-scale datasets \citep{chen2021learning, ma2023vip}. 
% The robot's reward $\rewr$ is unknown a priori and must be learned from human feedback.
% such as ImageNet \citep{deng2009imagenet}, R3M \citep{nair2022r3m}, or MVP \citep{xiao2022masked, radosavovic2023real}. 


% Thus, human feedback is precisely driven by this combination of their visual representation and their reward: $\uH \sim \policyh(\uH \mid \reph(\obs))$. \abnote{maybe when we introduce the human, we introduce them as providing preference feedback? the murky water here is that with our method, the human \textit{could} be the demonstrator, but they are \textit{also} the preference-based label-er.}

Before the robot can optimize for $\policyr$, it is faced with two questions: what visual representation $\repr$ should it use to encode observations, and which reward $\rewr$ should it optimize to align its behavior with $\policyh^{*}$?

% Unfortunately, both $\reph$ and $\rewh$ are unknown to the robot a priori. 

% \textbf{Dataset.} We assume the robot has access to a dataset of videos $\mathcal{D} = \{\obstraj_n\}^N_{n=0}$. For example, these could be obtained via roll-outs of an existing policy, the human performing teleoperation, or the human doing the task themselves. We do not make an assumption on if these videos are performed on the robot's embodiment or on a different embodiment, such as the human's. These videos will be used for both preference-based learning and for robot behavior alignment. \abnote{I'm not sure this should be here...but i felt like we need to somewhere mention that we get a dataset from which the robot learns the representation and the behavior alignment...}

% \abnote{\textbf{Note:} We could also have a subsection here on optimal transport as the reward structure? but it feels a bit premature...}

% In this work, we are interested in the setting where $\rewr$ is unknown to the robot and it must learn it from the human teacher. Moreover, we want to understand how the robot should build its visual representation $\rewr$ so that it can effectively?
% Ideally, the robot should optimize for the human's desired reward function, 
% i.e., $\rewr \equiv \rewh$, so the induced robot behavior optimizes for human preferences. 



% \item We model the robot's planning problem as a Markov decision process (MDP), $<\mathcal{O}, \repr, U_\mathrm{R}, T, \rewr, \gamma>$ where $\repr: \mathcal{O} \rightarrow \Phi_{\mathrm{R}}$ is the robot's visual representation model that maps the perceptual input to a latent representation space $\Phi_{\mathrm{R}}$, the transition function is $T(\obs^t,\uR^t, \obs^{t+1}): \mathcal{O} \times U_\mathrm{R}\times \mathcal{O} \rightarrow [0,1]$, $\rewr(\repr(\obs)): \Phi_{\mathrm{R}} \rightarrow \mathbb{R}$ is the robot's reward function and $\gamma \in (0,1]$ is the discount factor. The robot seeks an optimal policy $\pi^*_\mathrm{R}$ which maximizes the expected total reward:
% \begin{equation}
% \begin{aligned}
% \policyr^* = \arg\max_{\policyr}  \mathbb{E}_{}\Big[ \sum_{t=0}^{\infty} \rewr(\obs^t)\Big].
% \end{aligned}
% \label{eq:robot_planning_problem}
% \end{equation}





==> old_sections/sim_environments.tex <==
\subsection{Simulation Environments}
\label{subsec:experiment setup}


\begin{wrapfigure}{r}{0.45\textwidth}
    \vspace{-0.5cm}
    \includegraphics[width=0.45\textwidth]{figs/sim_environments.png}
    \vspace{-0.8cm}
  \caption{X-Magical and IsaacGym tasks.}
  \vspace{-0.5cm}
  \label{fig:x-magical-env}
\end{wrapfigure}

\subsubsection{X-Magical} 
\label{subsubsec:xmagical-setup}
\textbf{Tasks.} We first use the toy simulation environment, X-Magical \citep{zakka2022xirl}. We consider two tasks inspired by kitchen countertop cleaning. The robot always has to push objects to a goal region (e.g., trash can), shown in pink at the top of the scene in \autoref{fig:x-magical-env}. In the \textbf{avoiding} scenario, the end-user prefers that the robot and objects never enter an \textit{off-limits zone} during pushing (blue box in left \autoref{fig:x-magical-env}).
% where the robot needs to push the object (red square) towards a static goal region (light red region) without entering a disfavored region (light blue region). 
In the \textbf{grouping} scenario, the end-user prefers that objects are always pushed \textit{efficiently together} towards the goal region (center, \autoref{fig:x-magical-env}).

\textbf{Privileged State \& Reward.}
For \textbf{avoiding}, the true state $s$ is 7D: planar robot position ($p_\robot \in \mathbb{R}^2$) and orientation ($\theta_\mathrm{R}$),  planar position of the object ($p_{\mathrm{obj}}\in \mathbb{R}^2$), distance between goal region and object, ($d_{\mathrm{obj2goal}}$), and distance between the off-limits zone and the object ($d_{\mathrm{obs2obj}}$). The human's reward is: $\rewh_{\mathrm{avoid}}(s) = - d_{\mathrm{goal2obj}} - 2\cdot \mathbb{I}(d_{\mathrm{obs2obj}} < d_{\mathrm{safety}})$,
For \textbf{grouping}, the state is 9D: $s := (p_\robot, \theta_\robot$, $p_{\mathrm{obj^1}}, p_{\mathrm{obj^2}}, d_{\mathrm{goal2obj^1}}$, $d_{\mathrm{goal2obj^2}})$. The human's reward is: $\rewh_{\mathrm{group}}(s) = - \max(d_{\mathrm{goal2obj^1}}, d_{\mathrm{goal2obj^2}}) - ||p_{\mathrm{obj^1}} - p_{\mathrm{obj^2}}||_2$.
% : $(p_{\mathrm{R}}$, $\theta_\mathrm{R}$, $p_{\mathrm{obj^1}}$, $p_{\mathrm{obj^2}}$, $d_{\mathrm{goal2obj^1}}$ and $d_{\mathrm{goal2obj^2}}$.

% The human's \textbf{avoiding} 
% and for tabletop \textbf{grouping} .

\subsubsection{Robot manipulation} 
\label{subsubsec:manipulation-setup}
\textbf{Task.} We further validate our method in a robot manipulation task in the IsaacGym physics simulator \citep{makoviychuk2021isaac}. We implement the tabletop \textbf{grouping} task, where a robotic arm needs to learn to push two objects \textit{efficiently together} to the end-user's goal region (light blue region in right of \autoref{fig:x-magical-env}). 

\textbf{Privileged State \& Reward.}
The state $s$ is 16D: robot proprioception ($\theta_{\mathrm{joints}}\in \mathbb{R}^{10}$), 3D object positions
($p_{\mathrm{obj^{1,2}}}$), and object distances to goal ($d_{\mathrm{goal2obj^{1,2}}}$). The \textbf{grouping} reward is identical as in Section~\ref{subsubsec:xmagical-setup}. 

